Universal Source Separation with Weakly Labelled Data

Universal source separation (USS) is a fundamental research task for computational auditory scene analysis, which aims to separate mono recordings into individual source tracks. There are three potential challenges awaiting the solution to the audio source separation task. First, previous audio source separation systems mainly focus on separating one or a limited number of specific sources. There is a lack of research on building a unified system that can separate arbitrary sources via a single model. Second, most previous systems require clean source data to train a separator, while clean source data are scarce. Third, there is a lack of USS system that can automatically detect and separate active sound classes in a hierarchical level. To use large-scale weakly labeled/unlabeled audio data for audio source separation, we propose a universal audio source separation framework containing: 1) an audio tagging model trained on weakly labeled data as a query net; and 2) a conditional source separation model that takes query net outputs as conditions to separate arbitrary sound sources. We investigate various query nets, source separation models, and training strategies and propose a hierarchical USS strategy to automatically detect and separate sound classes from the AudioSet ontology. By solely leveraging the weakly labelled AudioSet, our USS system is successful in separating a wide variety of sound classes, including sound event separation, music source separation, and speech enhancement. The USS system achieves an average signal-to-distortion ratio improvement (SDRi) of 5.57 dB over 527 sound classes of AudioSet; 10.57 dB on the DCASE 2018 Task 2 dataset; 8.12 dB on the MUSDB18 dataset; an SDRi of 7.28 dB on the Slakh2100 dataset; and an SSNR of 9.00 dB on the voicebank-demand dataset. We release the source code at https://github.com/bytedance/uss

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> old.tex <==
In this work, we will focus on the separation 


The source separation problem is difficult when a recording is mono, where the problem turns into underdetermined. 

Source separation is closely related with computational auditory scene analysis (CASA). 

Source separation is also a well know task of cocktail party problem. Source separation is famous for being a cocktail party problem, where all sounds are mixed together. The difficulty comes from that we aim to separate them from a single channel source. 

Recently, there is a task called computational auditory scene analysis, which is a task to separate all sources from mixtures. Different from conventional source separation methods, the CASA system aims to separate everything, which is a challenging task. The CASA has been investigated for several years, while the progress is not very fast. The main reason is that the target to be separate is very complicated. 

for example, fully connected neural networks are used on the spectrogram of an audio recording, where the regression is learnt to separate the masks or linear spectrogram of audio sources. Convolutional neural networks are a kind of neural network that is orginated from image classification, where the convllutional kernels are used to extract high level features from the spectrogram. CNNs have also been shown to perform well on the source separation task. A kind of cnn is UNET originated from biological image segmentation, where the different hierarchy of feature maps are concatenated from different hierarchy to fully utilitze the different level information of spectrograms. Recurrent neural networks are kinds of neural networks that are able to capture long time temporal information of time domain sequences. Especially the spectrogram on the time domain. Recently, time-domain neural networks have been proposed for solving the source separation task, such as the TASNET architecture. The motivation is that the fourier transform may not be the optimal representation of audio signals. So time domain representation is a more natrual way to represent audio signals.

Datasets are important for building source separation systems. Previous works have used strongly labelled datasets such as VOICEBANK, musdb18, fsd datasets etc. for buidling source separation systesm. However, the collection of clean datasets can be difficult and time consuming. Recently, a large-scale dataset called AudioSet is proposed includes a large-scale amount of sound classes. including 527 sound classes with 2 million 10-second audio clips. The dataset covers a wide range of sounds with ontology, and has been widely used for audio classification and sound event detection tasks. 

Universal source separation have attracted several interests in recent years. For example, the Google proposed a universal source separation architecture for building the universal source separation system. The system applies a PIT criteria for separating signals in an unsupervised way. Later mix of mixture models are proposed for building the source separation system in an unsupervised way that can use mixture signals as input. There are several ways for building the general source separation system. In xxx, a weakly labelled system is trained on the AudioSet to build source separation systems. To begin with, sound event detection systems are proposed to detect the possible sound events in an audio recording. Then, source separation neural networks use those conditions to separate audios from different sound classes. The condition controls what sounds to be separated. Previous work initially investigated the source separation with those systems. Other works of universal source separation includes using query for budilding source separation systems. For example, training a zero-shot query based source separation system. 

However, there is a lack of research on investigating the general source separation with a large-scale. This paper is an extension of our previously proposed weakly labelled supervised source separation system. The contribution includes: 1) Use large-scale AudioSet for budiling general source seapration system: 2) Investigate music source separation, speech enhancement, and general sound separation with weakly labelled data 3) Investigate ontology based source separation system. 4) We combine source separation, sound event detection and audio tagging into a single system. 

This paper is organized as follows, Section I introduces neural network based source separation methods. Section 2 introduces our proposed universal source separation methods. Section 3 introduces ontology based separation. Section 4 shows experiments. Section 5 Concludes and forcast this work. 

\subsection{Weakly labelled audio data}
Previous audio tagging, sound event detection and source separation works mostly use strongly labelled data for training. Strongly labelled data means that there are clean sources or clean labels for training. However, the amount of training data can be limited with strongly labelled data, because the labelling of them can be time consuming. Therefore, recently, there are several work investigating audio tagging, sound event detection and source separation with weakly labelled data. We formally define the weakly labelled data problem as follows:

We denote the waveform of an audio clip as $ x \in {\mathbb{R}}^{L} $, where $ L $ is the length of the audio clip. Then the weak label of the audio clip is denoted as $ y \in {0, 1}^{K} $, where $ K $ is the number of sound classes in the audio clip, where $ 1 $ indicates the presence of sound class in the audio clip, and $ 0 $ indicates the absence of sound class in the audio clip. There are no time information, nor clean speech of signals in the audio clip. Though, our final target is to separate the source signals from the mixture even if there are no clean sources for training.

Source separation with weakly labelled data has been researched since 2019, and there are several ways to implement this. In this paper, we continue our system that combines the audio tagging, sound event detection and source separation system together. The framework of the proposed system is shown in Fig. \ref{}. The difficulty of the training of source separation system comes from that there are no clean sources for training, and all sources are mixture. To begin with, the audio tagging, sound event detection and source separation systems are trained separately. 


For the weakly labelled AudioSet, each audio clip is labelled as the presence or absence of sound classes, but not their occurrance time. Our first time is trying to locate the occurrance time of those sound events. One challenge of our proposed system is training a sound event detection system with weakly labelled data. Previous works have investigated using weakly labelled trianing methods. We adopt those methods to find the most likely part of an audio segment that likely to contain the sound events. That is, we learn a mapping to obtain the SED result on each segment $ x_{m} $:

\begin{equation} \label{eq1}
f(x_{m}): x_{m} \mapsto y
\end{equation}

Then the clip level prediction can be obtained by an aggregation function:

\begin{equation} \label{eq1}
F(x) = \text{agg}(\{f_{m}\}_{m=1}^{M})
\end{equation}
\noindent where $ M $ is the number of segments in an audio clip. Therefore, the system can be trained in an end-to-end method. After training, in the inference stage, given and audio clip, we can calculate its SED prediction by $ f(x_{m}) $. Therefore, by the SED system we can choose the segment that most likely to contain sound events for training the source separation system. The SED system can be modeled by a neural network, such as convolutional neural network.


The reason we do not use the entire 10-second audio clip for training the source separation system is that, some sound classes can be very short, such as gun shot, etc. Therefore we need to use very short segments that are most likely to contain sound events. Usually the duration of the short segments of 2 second or 3-seoncd is a good choice. After obtaining the anchor segments, we need to predict what sound events are there in the anchor segment. Although we could use the SED system in equation \ref{} to predict the audio tagging results. However, we found that the audio tagging result obtained from the SED system is not as good as building an audio tagging system from scratch. That is, we do not need SED system for audio tagging. So we build an audio tagging system as follows. 

\begin{equation} \label{eq1}
f(x): x \mapsto y
\end{equation}




\noindent where $ x $ is the entire audio clip, and $ y $ is the weak label of an audio clip. Instead of using any intermeidate representations, we model the $ f $ using a convlutional neural network that can be trained without using SED results. We use PANNs architecture to build the audio tagging system. In inference, we input the $ f $ with an anchor segment, and predict the audio tagging result as the predicted sound events in this audio clip. 


However, the main difficulty of training (\ref{eq:cond_ss_f}) is that there are 


\noindent where the function $ f $ can be modeled by neural networks. For example, fully connected neural networks, recurrent neural networks or convolutional neural networks. The DenseNet has ahcieved the top-1 perofmrance on MUSDB18 separation task. Usually, a time-domain waveform is extracted spectrogram by using short time Foureir transforms (STFT). Then, neural networks can be built on the spectrogram to separate signals. For example, the UNet takes the magnitude spectrogram as input and output separated spectrogram of sources. In \cite{}, we proposed a very deep UNet complex system for source separation, and achieved the state of the art performance on music source separation. the system can be written as:

\begin{equation} \label{eq1}
f: |X| \mapsto |S|.
\end{equation}


\noindent We denote the angle of mixture as $ \Theta_{\text{mix}} $, and the angle of $ s $ as $ \Theta_{\text{tar}} $. Our system predicts the incremental of angle $ \Theta_{\Delta} $. So that $ \Theta_{\text{mix}} = \Theta_{\text{tar}} + \Theta_{\Delta} $. Then, we have:
\begin{equation} \label{eq1}
\begin{split}
\hat{S} &= |\hat{S}| e^{\angle j\Theta_{\text{tar}}} \\
&= |\hat{S}|(\text{cos} \Theta_{\text{tar}} + j \text{sin} \Theta_{\text{tar}}) \\
&= |\hat{S}|(cos (\Theta_{\text{tar}} + \Theta_{\Delta}) + j sin (\Theta_{\text{tar}} + \Theta_{\Delta})) \\
&= |\hat{S}|(cos \Theta_{\text{tar}} cos \Theta_{\Delta} - sin  \Theta_{\text{tar}} sin \Theta_{\Delta} + j sin \Theta_{\text{tar}} cos \Theta_{\Delta} + j cos\Theta_{\text{tar}} sin \Theta_{\Delta})
\end{split}
\end{equation}

\noindent where
\begin{equation} \label{eq1}
cos \Theta_{\text{tar}} = \hat{S}_{\text{real}} / |\hat{S}|
\end{equation}

\noindent where the angle can be calculated by

\begin{equation} \label{eq1}
sin \Theta_{\text{tar}} = \hat{S}_{\text{imag}} / |\hat{S}|
\end{equation}

\noindent and the system will predict the real and imaginary part of predicted spectrogram.

\begin{equation} \label{eq1}
f: X \mapsto S_{\text{real}}
\end{equation}
\begin{equation} \label{eq1}
f: X \mapsto S_{\text{imag}}
\end{equation}

\noindent To begin with, we calcualte 

In addition to the spectrogram domain systems, there are time-domain source separation systems such as TasNet, where the models are built on the waveforms directly without modeling the STFT transforms. The time domain source separation systems have been widely explored in recently years. While we use spectorgram based systems bcause of their good performance. 

\begin{figure*}[t]
  \centering
  \centerline{\includegraphics[width=\textwidth]{figs/framework.pdf}}
  \caption{Confusion matrix of event based accuracy in Task 1.}
  \label{fig:results}
\end{figure*}


\subsection{Source separation}
Then, we come to the part to build a universal source separation system. Though we have selected anchor segments that most likely to contain sound events, there are still no information where the sound events appear in the audio clips, nor the clean sources of them. To tackle this problem, we propose a conditional based method to separate arbitrary sound classes given the sound class as a condition. To explain, we denote the anchor segment as $ x_{} $, and denote the condition of the sound source as $ c $. Then, our system is to build a regression:

\begin{equation} \label{eq1}
\hat{s} = f_{\text{sep}}(x_{1} + x_{2}, c_{1})
\end{equation}

\noindent, where $ x_{1} $ and $ x_{2} $ are two randomly selected anchor segments that contain disjoint sound classes. The condition $ c_{1} \in \mathbb{R}^{K} $ is a vector that controls what sounds to separate. For example, if $ c_{1} $ represents speech, then the separation result would be speech only. In training, each anchor segment is not clean, so that the condition is used to let the system know what sound events are there in the anchor segment $ x_{1} $. In inference, we manually set the conditional vector $ c_{1} $ to the sound classes we want to separate to obtain the separated sound classes. the advantage of our proposed method is that, during the entire training stage, there is no need of using strongly labelled data, and we can train the SS system with weakly labelled audios. 



\subsubsection{Loss functions}

asdf
\section{Universal source separation methods}
The universal source separation system relies on the choice of audio segments. For example, the anchor segments selected should be disjoint and there are no overlap between audio segments. Otherwise, there can be confusion effects when separating the two segments. To begin with, we propose a hard-example mining method to mine the audio segments that are disjoint. 

\subsection{Separation model}
To begin with, we introduce the source separation model we used in our experiments. As we found that UNet is a steady system for source separation, we adopt the unET as the basic source separation system. We dive the UNet into very deep separation neural network with up to 96 layers that is called ResUNet. To begin with, we extract spectrogram on the fly from waveforms with the torchlibrosa toolkit. Therefore our separation is purely end-to-end system. Then we build convolutional blocks with 6 encdoer layers, 4 intermediate convolutional layers, and 6 decoder layers as the separation system. Each encoder consists of 4 residual convolutional blocks. Each residual convolutional blaock consists of two convolutional layers, where each convolutional layer consists of a pre-bn, a leaky-relu nonlinearity and a convolutional operation. The reason we choose this combination is that there is an abn module in the system. Then, the average pooling is applied to each encoder layer Therefore, there are 6x4x2 layers in the encoder. For the intermediate convolutional layer, the convolutional operation is the same as encoder layer. So there are 4x4x2 layers in intermediate layers. For the decoder, it is symmetric to the encoder, where there transposed convolutional layer to upsample the feature maps to the original size of the spectrogram. Then the spectrogram as well as the predicted phase difference are used to reconstruct the original waveform signal as described in equation (\ref{}). 

\subsection{Hard example mining}
Hard example mining is an important part for building the geenral source separation model. For example, there can be 1 million audio clips containing speech and music in AudioSet. So randomly mix them may cause a problem that both of two anchor segments will contain speech. This is the phenomenon that our system try to avoid.  Therefore, we propose a hard example mining method for detecting the important anchor segments to be mixed. 

The most important part is that, we first select anchor segments from different sound classes. Because the weak labels from AudioSet may not cover every sound events in an audio clip. That is, there might be missing sound events in the labels. So we use the PANNs prediction as the label prediction. Then we predict the audio tags probabilities of the anchor segments. Then if the two anchor segment share the same sound class with highi probability, they they are abandonded. Otherwise if they are disjoint, then they are used as anchor segments. Then, those two anchor segments can be mixed into a mixture. The mixture is fed into the separation neural network to separate one of the sources. There is no need for the source to be separated to be clean. For example, the source to be separated can be mixture of sound classes. And the information to be separated is inside the condition. 

\subsection{Hard condition VS soft condition}
There are two different ways to build the condition. One is called hard condition, which means the conditional vectory is build with one-hot vectors with values of either 0 or 1. For example, the hard condition can be $ [0, 1, 0, 0, 1, 0, ...] $ Another way is called soft condition, where the conditions are built with the soft predictions of audio clips. The advantage of soft condition is that, there are flexibility of sound classes information to be separated. For example, the soft condition can be $ [0.1, 0, 5, 0.1, 0.2, ...] $. In training, we can build systems with either hard of soft training. In inference, we can also condition on the type of sound events we want to separate. In addition, the condition can be soft condition or hard condition. The advantage of hard condition is that, we already know what sound sources to separate and explicitly indicate the source we want to separate. On the other hand, the advantage of soft condition is that, we allow ambuiguity of different sound classes for building the separation system.

\subsection{embedding condition}
There is also a possibility that we can use embedding as condition as input to the neural networks instead of one hot encodings. The advantage of using embedding as conditional vector is that, we can do example based source separation. That is, we can do zero shot separation. We do not need to explicitly know what sound events we want to separate, but we just give an example. the embedding is calcualted from our audio tagging system, which is already pretrained. Therefore, we assume that the embedding contains sufficient information of what sound event it looks like. we denote the embedding as $ h_{\text{emb}} = g_{\text{AT}}(x) $, where $ h_{\text{emb}} $ is the embedding vector we want to input to the neural network as condition. We denote the separation system as 

\begin{equation} \label{eq:embedding}
f(x) = W * x + V h_{\text{emb}}
\end{equation}

\noindent where $ h_{\text{emb}} $ controls what sound event to separate. One difference from the embedding condition VS the one hot encdoing is that, we need to give an exmaple to calculate the embedding vector. In addition, the sound classes may have a multiple center distribution. For example, the Speech can be from different speakers. We ignore the difference between speakers, and average all speaker as one averaged speaker. But the advantage is that we can separate arbitrary sound events if there is an example. 


\section{}
\subsection{Percetpual loss functions}
we can train the neural network with several different kinds of loss functions. The most common loss function is the loss function on the spectrogram, which is also called spectrogram loss function. The loss function can be L1 or L2, corresponding to mean absolute error or mean squared error. The advantage of the spectrogram loss is that, it is correspond to human perception on sensing audio signals. Another type of loss function is called waveform domain L1 or L2 loss. the calculation of the waveform domain loss is on the time domain signal. And is more sensitive to the phase distrotion when doing the separation system. We denote the time-domain loss function as: $ s - \hat{s} $. 

According to \ref{}, there are several perceptual loss function that may not be directly modeled by this direct pixel-wise distance. Therefore, several vggish or high-level loss functions have been proposed. One of them is called GAN loss function, where the GAN is used to distinguish from real and fake samples. In our cases, GAN is used to separate the mixture source into independent sources that are difficult for the discriminator to classify. After this kind of training, we will get a good generator and a good discriminator. And the separation result can be good. 

\subsection{Unsupervised clustering separation}
One feature of the AudioSet dataset is that, there can be multiple sound classes with an ontology of 527 sound classes in its current version. the sound classes are not independent, and there is a tree hierarcy of the sound classes. For example, the Ambulence belongs to car, belongs to vehicle, etc. There are several ways to utilize this hierarchy information in building our system. 

\subssection{one-to-one mapping}
The first kind of mapping is called one-to-one mapping, where we only set one value of 1 to the sound classes to separate. For example, for speech separation, we take the speech sound class to build the one-hot vector as condition. This one-to-one mapping is simple and easy to implement. While there can be some specific cases, such as when separating femal speech, it is indeed belongs to speech and should be separated. Therefore we propose hierarchy separation. 

\subsection{hierarchy separation}
The AudioSet ontology contains 7 root sound classes, including human sounds, music, etc. One possible one is to group the sound classes into major sound classes, that can be separated into different sound classes. Also, there can be the second level categories, and third level categories, etc. The advantage of using the ontology separation is that, we can confidently separate the sound classes into different categories. 


Fig. \ref{} shows the class-wise separation result of all sound classes from AudioSet. 

AudioSet is a large-scale dataset includes 2 million 10-second audio clips. The audio clips of AudioSet is from YouTube. And the audio clips are from real recordings. Therefore the distribution of AudioSet is the same as the sounds in the world. There are 527 sound classes in the current version of AudioSet. And the sound classes have an ontology. AudioSet is weakly labelled, that is, we only know the presence or absence of sound events in the dataset, but not the precise onset and offset time of sound events. Let along the separated sources. To build the conditional vector for our source separation system, we use PANNs. To evaluate the class-wise separation performance, we calcualte their SDR result. Figure xxx shows the overall SDR of the balanced and full dataset with different iterations. The training can be quite slow due to the large amount of sound events. Fig. xxx shows the full SDR result of all sound classes, which is a long figure. From those figures, we show that the separation ability of different sound classes can be different. Some sound classes are easier to separate, while others are more difficult. Table xx shows the SDRis of seven major sound classes of AudioSet. A detailed long figure of all 527 sound classes can be seen in Fig. xxx. 


We first evaluate our system with the speech enhancement dataset, especially the voiceband-demand dataset. The voiceband-demand datasets consists of 10000+ speech and xxx+ background noise in their training set. We propose to build our system on this dataset with weakly labelled data. the evaluation criteria includes pesq, covl, ssnr etc. To begin with, we build strongly labelled systems. Then, we compare the strongly labelled system with AudioSet based systems. 

\begin{table}[t]
\centering
\caption{SED on DESED}
\label{table:sed}
\begin{tabular}{*{8}{c}}
 \toprule
 & PSDS 0.1 & PSDS 0.5 & PSDS 0.7 & Collar-based \\
 \midrule
 CNN Max & 0.480 & 0.425 & 0.083 & 0.040 \\
 CNN Att & 0.485 & 0.459 & 0.066 & 0.040 \\
 HTS \\
 \bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{SED on 381}
\label{table:sed}
\begin{tabular}{*{8}{c}}
 \toprule
 & PSDS 0.1 & PSDS 0.5 & PSDS 0.7 & Collar-based \\
 \midrule
 CNN Max \\
 CNN Avg \\
 CNN Decision \\
 HTS \\
 \bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{UNet soft condition}
\label{table:is_baseline}
\begin{tabular}{*{5}{c}}
 \toprule
 & SDRi & SI-SDRi & ME SDRi & ME SI-SDRi \\
 \midrule
 mixture & 0 & 0 & 0 & 0 \\
 \midrule
 WavUNet \\
 ConvTasNet \\
 UNet \\
 UNetComplex \\
 DeepReisudalUNet \\
 SubbandResNet \\
 \bottomrule
\end{tabular}
\end{table}


======================

Weakly labelled datasets contain audio clips with tags, while there are no information when the tags occur. Each audio clip may also contain interference sounds. 

\begin{table*}
  \caption{Balanced VS Full set}
  \label{tab:result}
  \centering
  \begin{tabular}{lccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{AudioSet}} & \multicolumn{2}{c}{\textbf{DCASE2018 Task2}} & \multicolumn{2}{c}{\textbf{FSD50k}} & \multicolumn{2}{c}{\textbf{Musdb18}} & \multicolumn{2}{c}{\textbf{Slakh2100}} & \multicolumn{2}{c}{\textbf{VoicebankDemand}} \\
	\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    & ora. emb & avg. emb & SDRi & SISDRi & SDRi & SISDRi & SDR & wi-SDR & SDRi & SISDRi & PESQ & SSNR  \\
    \midrule
    Balanced (200k) & 7.76 & 5.45 & 9.63 & 7.02 & 5.34 & 0.66 & 2.39 & & 7.02 & 3.37 & 2.35 & 8.10 \\
    Balanced (600k) & 8.35 & 5.60 & 10.61 & 7.76 & 5.49 & -0.25 & 2.88 & & 7.47 & 3.78 & 2.46 & 11.07 \\
    Balanced (2000k) & 8.59 & 5.52 & 11.04 & 8.40 & 5.56 & -0.55 & 2.59 & & 7.45 & 4.02 & 2.41 & 10.42 \\
    Full bal (nobal tr. 600k) & 8.41 & 6.09 & 10.89 & 8.63 & 5.95 & 0.89 & 2.52 & & 6.84 & 4.00 & 2.30 & 11.19 \\
    Full bal (nobal tr. 2000k) & 9.01 & 6.73 & 12.34 & 10.82 & 6.97 & 2.44 & 1.52 & & 5.84 & 3.80 & 2.42 & 11.03 \\
    Full bal (bal tr. 600k) & 8.44 & 6.34 & 10.91 & 8.74 & 6.15 & 1.10 & 2.30 & & 6.66 & 3.81 & 2.45 & 11.00 \\
    Full bal (bal tr. 2000k) & 9.10 & 6.60 & 12.57 & 10.60 & 6.95 & 2.31 & 2.71 & & 6.33 & 3.80 & 2.37 & 11.18 \\
    Full bal (bal tr. 600k, bs=4) & 9.45 & 6.76 & 12.54 & 10.26 & 7.13 & 1.88 & 2.80 & & 6.12 & 3.86 & 2.57 & 11.79 \\
    Full bal (bal tr. 2000k, bs=4) & 9.93 & 7.21 & 14.49 & 12.59 & 7.79 & 2.88 & 2.16 & & 5.31 & 4.00 & 2.49 & 11.82\\
    
    \bottomrule
\end{tabular}
\end{table*}

\begin{table*}
  \caption{Embeddings}
  \label{tab:result}
  \centering
  \begin{tabular}{lccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{AudioSet}} & \multicolumn{2}{c}{\textbf{DCASE2019 Task2}} & \multicolumn{2}{c}{\textbf{FSD50k}} & \multicolumn{2}{c}{\textbf{Musdb18}} & \multicolumn{2}{c}{\textbf{Slakh2100}} & \multicolumn{2}{c}{\textbf{VoicebankDemand}} \\
	\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    & ora. emb & avg. emb & SDRi & SISDRi & SDRi & SISDRi & SDR & wi-SDR & SDRi & SISDRi & PESQ & SSNR  \\
    \midrule
    onehot & 5.90 & 5.90 & 7.94 & 5.64 & 5.76 & 3.14 & & & - & - & 2.29 & 5.36 \\
    segment-prediction & 7.33 & 6.20 & 9.16 & 7.10 & 5.94 & 2.71 & 2.41 & &  5.33 & 2.52 & 2.46 & 10.10 \\
    embedding & 8.35 & 5.60 & 10.61 & 7.76 & 5.49 & -0.25 & 2.88 & & 7.47 & 3.78 & 2.46 & 11.07 \\
    \bottomrule
\end{tabular}
\end{table*}

\begin{table*}
  \caption{Segment seconds}
  \label{tab:result}
  \centering
  \begin{tabular}{lccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{AudioSet}} & \multicolumn{2}{c}{\textbf{DCASE2019 Task2}} & \multicolumn{2}{c}{\textbf{FSD50k}} & \multicolumn{2}{c}{\textbf{Musdb18}} & \multicolumn{2}{c}{\textbf{Slakh2100}} & \multicolumn{2}{c}{\textbf{VoicebankDemand}} \\
	\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    & ora. emb & avg. emb & SDRi & SISDRi & SDRi & SISDRi & SDR & wi-SDR & SDRi & SISDRi & PESQ & SSNR  \\
    \midrule
    0.5 s & 5.20 & 3.73 & 4.35 & -2.37 & 2.63 & -5.62 & 1.91 & & 6.83 & 1.52 & 1.82 & 8.09\\
    1s & 7.76 & 5.37 & 8.38 & 5.61 & 4.61 & -0.77 & 1.58 & & 6.87 & 3.54 & 2.13 & 8.86 \\
    2s & 7.76 & 5.45 & 9.63 & 7.02 & 5.34 & 0.66 & 2.39 & & 7.02 & 3.37 & 2.35 & 8.10 \\
    4s & 6.92 & 4.94 & 8.04 & 6.07 & 4.63 & 0.38 & 0.89 & & 4.79 & 2.78 & 2.45 & 8.48 \\
    6s & 6.17 & 4.44 & 6.31 & 3.18 & 3.95 & -1.50 & -0.57 & & 4.16 & 1.95 & 2.20 & 5.23 \\
    8s & 5.96 & 4.32 & 7.10 & 4.68 & 4.33 & -0.37 & -1.15 & & 2.69 & 1.73 & 2.39 & 7.88 \\
    10s & 6.02 & 4.42 & 6.92 & 4.26 & 4.23 & -0.36 & -1.47 & & 2.58 & 1.38 & 2.43 & 5.67 \\
    \bottomrule
\end{tabular}
\end{table*}

\begin{table*}
  \caption{Segment seconds}
  \label{tab:result}
  \centering
  \begin{tabular}{lccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{AudioSet}} & \multicolumn{2}{c}{\textbf{DCASE2019 Task2}} & \multicolumn{2}{c}{\textbf{FSD50k}} & \multicolumn{2}{c}{\textbf{Musdb18}} & \multicolumn{2}{c}{\textbf{Slakh2100}} & \multicolumn{2}{c}{\textbf{VoicebankDemand}} \\
	\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    & ora. emb & avg. emb & SDRi & SISDRi & SDRi & SISDRi & SDR & wi-SDR & SDRi & SISDRi & PESQ & SSNR  \\
    \midrule
    SED 2s & 7.76 & 5.45 & 9.63 & 7.02 & 5.34 & 0.66 & 2.39 & & 7.02 & 3.37 & 2.35 & 8.10 \\
    random 2s & 7.62 & 5.56 & 8.92 & 6.30 & 5.11 & 0.24 & 1.89 & & 6.58 & 2.55 & 2.33 & 8.93\\
    self 2s & 3.95 & 3.22 & 4.46 & 2.49 & 3.25 & 0.18 & 0.74 & & 6.27 & 1.61 & 2.10 & 6.81 \\
    avoid conflict \\
    \bottomrule
\end{tabular}
\end{table*}

\begin{table*}
  \caption{Audio Tagging mAP 20k}
  \label{tab:result}
  \centering
  \begin{tabular}{lccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{AudioSet}} & \multicolumn{2}{c}{\textbf{DCASE2019 Task2}} & \multicolumn{2}{c}{\textbf{FSD50k}} & \multicolumn{2}{c}{\textbf{Musdb18}} & \multicolumn{2}{c}{\textbf{Slakh2100}} & \multicolumn{2}{c}{\textbf{VoicebankDemand}} \\
	\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    & ora. emb & avg. emb & SDRi & SISDRi & SDRi & SISDRi & SDR & wi-SDR & SDRi & SISDRi & PESQ & SSNR  \\
    \midrule
    Random & 7.68 & 2.94 & 5.12 & -2.77 & 2.53 & -8.64 & -0.24 & & 6.78 & -2.68 & 1.85 & 3.71 \\
    Cnn6 & 8.27 & 5.26 & 9.04 & 6.09 & 4.78 & -0.81 & 3.08 & & 7.52 & 3.41 & 2.40 & 8.17 \\
    Cnn10 & 7.81 & 5.36 & 9.24 & 6.64 & 5.30 & 0.78 & 2.43 & & 7.11 & 3.65 & 2.45 & 8.78 \\
    Cnn14 & 7.76 & 5.45 & 9.63 & 7.02 & 5.34 & 0.66 & 2.39 & & 7.02 & 3.37 & 2.35 & 8.10 \\
    HTSAT (random) & 6.63 & 2.83 & 5.41 & 2.13 & 2.72 & -3.46 & 1.00 & & 8.23 & -0.40 & 2.22 & 2.80 &  \\
    HTSAT & 8.72 & 4.18 & 8.01 & 4.17 & 3.90 & -2.51 & 2.79 & & 8.39 & 3.40 & 2.39 & 6.76 \\
    \bottomrule
\end{tabular}
\end{table*}

\begin{table*}
  \caption{Audio types}
  \label{tab:result}
  \centering
  \begin{tabular}{lccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{AudioSet}} & \multicolumn{2}{c}{\textbf{DCASE2019 Task2}} & \multicolumn{2}{c}{\textbf{FSD50k}} & \multicolumn{2}{c}{\textbf{Musdb18}} & \multicolumn{2}{c}{\textbf{Slakh2100}} & \multicolumn{2}{c}{\textbf{VoicebankDemand}} \\
	\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    & ora. emb & avg. emb & SDRi & SISDRi & SDRi & SISDRi & SDR & wi-SDR & SDRi & SISDRi & PESQ & SSNR  \\
    \midrule
    
    Cnn14 & 7.76 & 5.45 & 9.63 & 7.02 & 5.34 & 0.66 & 2.39 & & 7.02 & 3.37 & 2.35 & 8.10 \\
    wav2vec & 8.43 & 4.71 & 8.30 & 5.36 & 4.52 & -0.84 & 1.93 & & 7.65 & 3.41 & 2.43 & 5.03 \\
    speaker & 8.08 & 2.96 & 6.61 & 2.01 & 3.46 & -3.55 & 1.40 & & 8.34 & 1.91 & 2.37 & 8.95 \\
    \bottomrule
\end{tabular}
\end{table*}


\begin{table*}
  \caption{Embeddings}
  \label{tab:result}
  \centering
  \begin{tabular}{lccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{AudioSet}} & \multicolumn{2}{c}{\textbf{DCASE2019 Task2}} & \multicolumn{2}{c}{\textbf{FSD50k}} & \multicolumn{2}{c}{\textbf{Musdb18}} & \multicolumn{2}{c}{\textbf{Slakh2100}} & \multicolumn{2}{c}{\textbf{VoicebankDemand}} \\
	\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    & ora. emb & avg. emb & SDRi & SISDRi & SDRi & SISDRi & SDR & wi-SDR & SDRi & SISDRi & PESQ & SSNR  \\
    \midrule
    freeze Cnn14 & 7.76 & 5.45 & 9.63 & 7.02 & 5.34 & 0.66 & 2.39 & & 7.02 & 3.37 & 2.35 & 8.10 \\
    \midrule
    learnable Cnn6 scratch & 9.67 & 2.23 & 2.99 & -2.28 & 2.22 & -8.21 & 2.43 & & 9.06 & 1.56 & 1.93 & 6.59 \\
    learnable Cnn14 scratch & 2.15 & 2.15 & 2.23 & -0.02 & 2.14 & -0.16 & -2.45 & & 2.82 & -0.00 & 2.19 & 1.19 \\
    - Conv1d scratch \\
    \midrule
    learnable Cnn14 mul task & 8.92 & 3.22 & 6.10 & 0.49 & 2.55 & -5.82 & 3.10 & & 8.80 & 3.99 & 1.89 & 6.84 \\
    \midrule
    freeze embedding + adaptor 1 \\
    freeze embedding + adaptor 2 & 7.78 & 5.86 & 10.05 & 7.71 & 5.91 & 1.25 & 2.58 & & 6.06 & 3.06 & 2.41 & 7.22 \\
    \midrule
    freeze residual Cnn6 & 7.52 & 5.20 & 8.78 & 6.00 & 4.85 & -0.40 & 2.46 & & 6.77 & 3.14 & 2.43 &  \\
    - freeze residual conv1d \\
    \bottomrule
\end{tabular}
\end{table*}

\begin{table*}
  \caption{Data augmentation}
  \label{tab:result}
  \centering
  \begin{tabular}{lccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{AudioSet}} & \multicolumn{2}{c}{\textbf{DCASE2019 Task2}} & \multicolumn{2}{c}{\textbf{FSD50k}} & \multicolumn{2}{c}{\textbf{Musdb18}} & \multicolumn{2}{c}{\textbf{Slakh2100}} & \multicolumn{2}{c}{\textbf{VoicebankDemand}} \\
	\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    & ora. emb & avg. emb & SDRi & SISDRi & SDRi & SISDRi & SDR & wi-SDR & SDRi & SISDRi & PESQ & SSNR  \\
    \midrule
    match energy & 7.76 & 5.45 & 9.63 & 7.02 & 5.34 & 0.66 & 2.39 & & 7.02 & 3.37 & 2.35 & 8.10 \\
    no aug & 6.69 & 3.94 & 6.87 & 3.74 & 3.64 & -2.46 & 1.76 & & 7.94 & 3.07 & 2.27 & 4.70 \\
    +-20 db & 3.96 & 3.02 & 2.97 & 0.65 & 1.94 & -2.29 & 0.09 & & 7.15 & 2.36 & 2.32 \\
    50\% & 7.26 & 4.56 & 7.89 & 5.16 & 4.11 & -1.46 & 1.40 & & 7.19 & 3.55 & 2.41 & 6.69 \\
    \bottomrule
\end{tabular}
\end{table*}


\begin{table*}
  \caption{Mix Type}
  \label{tab:result}
  \centering
  \begin{tabular}{lccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{AudioSet}} & \multicolumn{2}{c}{\textbf{DCASE2019 Task2}} & \multicolumn{2}{c}{\textbf{FSD50k}} & \multicolumn{2}{c}{\textbf{Musdb18}} & \multicolumn{2}{c}{\textbf{Slakh2100}} & \multicolumn{2}{c}{\textbf{VoicebankDemand}} \\
	\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    & ora. emb & avg. emb & SDRi & SISDRi & SDRi & SISDRi & SDR & wi-SDR & SDRi & SISDRi & PESQ & SSNR  \\
    \midrule
    2 to 1 & 7.76 & 5.45 & 9.63 & 7.02 & 5.34 & 0.66 & 2.39 & & 7.02 & 3.37 & 2.35 & 8.10 \\
    3 to 1-2 & 6.04 & 4.03 & 4.66 & 1.65 & 2.88 & -2.26 & 2.96 & & 7.51 & 2.92 & 2.10 & 5.59 \\
    4 to 1-3 & 5.14 & 3.49 & 3.97 & 1.37 & 2.45 & -1.81 & 1.63 & & 6.97 & 2.31 & 1.85 & 5.40 \\
    \bottomrule
\end{tabular}
\end{table*}

\begin{table*}
  \caption{Separation models}
  \label{tab:result}
  \centering
  \begin{tabular}{lccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{AudioSet}} & \multicolumn{2}{c}{\textbf{DCASE2019 Task2}} & \multicolumn{2}{c}{\textbf{FSD50k}} & \multicolumn{2}{c}{\textbf{Musdb18}} & \multicolumn{2}{c}{\textbf{Slakh2100}} & \multicolumn{2}{c}{\textbf{VoicebankDemand}} \\
	\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    & ora. emb & avg. emb & SDRi & SISDRi & SDRi & SISDRi & SDR & wi-SDR & SDRi & SISDRi & PESQ & SSNR  \\
    \midrule
    UNet \\
    ResUNet 30 \\
    ResUNet 60 \\
    WavUNet \\
    Demucs \\
    ConvTasNet \\
    DPRNN \\
    BSRNN \\
    \bottomrule
\end{tabular}
\end{table*}

\begin{table}
  \caption{Slakh2100}
  \label{tab:result}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    & zero & scratch & ft ada & ft all \\
    \midrule
    1 shot & 7.32 & 8.35 & 8.97 & 8.97 \\
    5 shot & 7.44 & 8.23 & 9.84 & 9.82 \\
    50 shot & 7.45 & 9.03 & 10.18 & 10.31 \\
    full & 7.48 & 9.60 & 10.25 & 10.46 \\
    \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{DCASE2018 task2}
  \label{tab:result}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    & zero & scratch & ft ada & ft all \\
    \midrule
    1 shot & 5.26 & 0.56 & 5.31 & 5.31 \\
    5 shot & 7.16 & 3.04 & 7.16 & 7.16 \\
    50 shot & 9.34 & 3.42 & 9.46 & 11.38 \\
    full & 9.34 & 3.65 & 10.87 & 12.09 \\
    \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Musdb18}
  \label{tab:result}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    & zero & scratch & ft ada & ft all \\
    \midrule
    1 shot & 1.49 & -1.72 & 1.49 & 1.49 \\
    5 shot & 1.86 & 0.34 & 1.87 & 1.87 \\
    50 shot & 1.77 & 1.34 & 2.75 & 2.86 \\
    full & 1.82 & 2.84 & 3.46 & 3.97 \\
    \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Voicebank-demand}
  \label{tab:result}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    & zero & scratch & ft ada & ft all \\
    \midrule
    1 shot & 2.49 & 2.07 & 1.69 & 1.83 \\
    5 shot & 2.45 & 2.19 & 2.34 & 2.36 \\
    50 shot & 2.37 & 1.90 & 2.50 & 2.71 \\
    full & 2.11 & 2.58 & 2.55 & 2.58 \\
    \bottomrule
\end{tabular}
\end{table}

We use three different condition types including 1) oracle condition, 2) single condition of the ``Speech'' class and 3) the clustering classes related to Speech for inference. Table \ref{table:result_speech_enhancemen} shows the result of using different conditional vectors. The general source separation system achieves a PESQ of 2.273. 


%Music source separation is a task to separate a music recording into individual sources, such as vocals and accompaniment. Recently, several single-channel music source separation methods have been proposed, while they are all rely on clean data. We experiment the general source separation system on the MUSDB18 dataset \cite{rafii2017musdb18}, which includes 100 training tracks 50 testing tracks. Clean sources of vocals, bass, drums, and other are provided for training. Different from previous works use clean data from the training set to train the system, we directly apply the trained separation system trained on AudioSet for music source separation. We resample audio recordings from 44.1 kHz to 32 kHz in our general source separation system. After separation, audio signals are resampled back to 44.1 kHz for evaluation. SDR is used as the evaluation criterion. 

\subsection{AudioSet separation}
We evaluate the general source separation performance on the AudioSet dataset. The evaluation set includes 18,887 audio clips which covers all 527 sound classes. Each sound class has at least 59 audio samples for evaluation. As the audio clips from AudioSet are weakly labelled, there are no information when sound events happen. To create a mixture, we randomly mine anchor segments $ s_{1} $ and $ s_{2} $ described in Section \ref{}. Then, we create a mixture by $ x = s_{1} + s_{2} $. Different from training, we do not apply scale augmentation at inference. To construct the conditional vector $ c $, we apply 1) The oracle audio tagging prediction of $ s_{1} $ from PANNs, 2) one-hot encoding of the target sound class when selecting $ s_{1} $, 3) audio tagging probabilities of $ s_{1} $ multiply the one-hot encoding of the sound class in elementwise. We use signal-to-distortion ratio improvement (SDRi) \cite{vincent2006performance} and scale invariant SDRi (SI-SDRi) \cite{le2019sdr} to evaluate the separation performance. The SDR between a target signal $ s $ and an estimated signal $ \hat{s} $ as:

\begin{equation} \label{eq:sdr}
\text{SDR}(s, \hat{s}) = 10 \text{log}_{10} \left ( \frac{||s||^2}{||s - \hat{s}||^2} \right ).
\end{equation}

\noindent To evaluate how the separation system improves without separation, the SDRi is defined as the $ SDRi = \text{SDR}(s, \hat{s}) - \text{SDR}(s, x) $. To address the scaling problem of SDR. Recently, SI-SDR was proposed, and is calcualted by:

\begin{equation} \label{eq:sisdr}
\text{SDR}(s, \hat{s}) = 10 \text{log}_{10} \left ( \frac{||\alpha s||^2}{||\alpha s - \hat{s}||^2} \right ),
\end{equation}

\noindent where $ \alpha $ is calculated by $ \hat{s}^{T}s / ||s||^2 $. Table \ref{table:result_audioset} shows the SDR and SiSDR \cite{le2019sdr} of the macro average of sound classes. The universal source separation system achieves a SDRi of 7.95 dB, and the SI-SDRi is 6.13 dB. Fig. \ref{fig:audioset_long_fig} shows the all 527 sound classes separation performance. The separation performance of different sound classes vary. For example, some sound classes are over 20 dB, while other sound classes are within 3 dB. 

% \begin{table}[t]
% \centering
% \caption{AudioSet separation}
% \label{table:result_audioset}
% \begin{tabular}{*{6}{c}}
%  \toprule
%  & SDRi & SI-SDRi & \\
%  \midrule
%  oracle & 7.95 & 6.13 & 7.90 \\
%  one-hot & 2.92 \\
%  at-mul & & 2.15 \\
%  \bottomrule
% \end{tabular}
% \end{table}







Table \ref{table:result_mss} shows source separation performance of our systems. We use oracle condition, one-hot condition and cluster condition for inference. Without any training data, our system achieves SDR of 4.491 dB when conditioned on speech and singing. 



\subsection{Instruments separation}
violin, flute, ..., 11 instruments

\subsection{FUSS separation}
The Free Universal Sound Separation (FUSS) dataset \cite{wisdom2021s} is a corpus for experiments in separating mixtures of an unknown number of sounds from an open domain of sounds. The dataset consists of 23 hours of single-source audio data drawn from 357 classes. The FUSS data is sourced from the FSD50K dataset. There are 7,237 clips, 2,883 clips, and 2,257 clips for training, validation and evaluation. For each mixture, the number of sounds is chosen uniformly at random in the range of one to four. Every mixture contains zero to three foreground source events, and one background source. 

Table \ref{} shows the separation result


\begin{table}
  \caption{Slakh2100}
  \label{tab:result}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    & zero & scratch & ft ada & ft all \\
    \midrule
    1 shot & 7.32 & 8.35 & 8.97 & 8.97 \\
    5 shot & 7.44 & 8.23 & 9.84 & 9.82 \\
    50 shot & 7.45 & 9.03 & 10.18 & 10.31 \\
    full & 7.48 & 9.60 & 10.25 & 10.46 \\
    \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{DCASE2018 task2}
  \label{tab:result}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    & zero & scratch & ft ada & ft all \\
    \midrule
    1 shot & 5.26 & 0.56 & 5.31 & 5.31 \\
    5 shot & 7.16 & 3.04 & 7.16 & 7.16 \\
    50 shot & 9.34 & 3.42 & 9.46 & 11.38 \\
    full & 9.34 & 3.65 & 10.87 & 12.09 \\
    \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Musdb18}
  \label{tab:result}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    & zero & scratch & ft ada & ft all \\
    \midrule
    1 shot & 1.49 & -1.72 & 1.49 & 1.49 \\
    5 shot & 1.86 & 0.34 & 1.87 & 1.87 \\
    50 shot & 1.77 & 1.34 & 2.75 & 2.86 \\
    full & 1.82 & 2.84 & 3.46 & 3.97 \\
    \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Voicebank-demand}
  \label{tab:result}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    & zero & scratch & ft ada & ft all \\
    \midrule
    1 shot & 2.49 & 2.07 & 1.69 & 1.83 \\
    5 shot & 2.45 & 2.19 & 2.34 & 2.36 \\
    50 shot & 2.37 & 1.90 & 2.50 & 2.71 \\
    full & 2.11 & 2.58 & 2.55 & 2.58 \\
    \bottomrule
\end{tabular}
\end{table}

\subsection{YouTube}

Our another application is to to separate the movie files from Youtube into differnet sources. That is, we are able to separate the mixture movies into different tracks for visualization. For this probelm, the number of sound events to be separated is unknown. Therefore, we need to design a strategy for building the separation system into different sources. We propose several cluster based categories for building the source separation system. 

\subsubsection{Category into root sound classes}
The first strategy is to category the sound classes into different root sound classes including Music, Human sounds, etc. The root representation can be parsed from the AudioSet ontology. For example, all human activity sounds including speech, vocals, clean throat will be categorized into human activities. In addition, music can be categorized into Africa music, european music and so on. The start of our research is to classify the sound events into 7 categories. 

There are also two ways of separating sounds. The first is directly separate whatever sound events in an audio clip based on their SED results. However, sometimes we find that even if the soft condition is all zero, then the separated sounds are not clean. So we design a second strategy, where SED is used to detect the presence or absence of sound classes. Then separation is only exectued on the segments where the SED prediction is over a certein threshold. We set the segments into silence if the SED prediction is lower than some threshold. 

\subsubsection{Category into sub-category sound classes}
We investigate our system that applies the separation into sub-categories. The layer of sound classes to be separate range from 1 to 5, with increased number of sound classes. 

\begin{table}[t]
\centering
\caption{AudioSet tagging results}
\label{table:sed}
\begin{tabular}{cccc}
 \toprule
 & mAP & mAUC & d-prime \\
 \midrule
 Random Guess & 0.005 & 0.500 & 0.000 \\
 AudioSet Baseline \cite{gemmeke2017audio} & 0.314 & 0.959 & 2.452 \\
 TAL Net \cite{wang2019comparison} & 0.362 & 0.965 & 2.554 \\
 DeepRes \cite{ford2019deep} & 0.392 & 0.971 & 2.682 \\
 \textbf{Cnn14 (PANN)} \cite{kong2020panns} & 0.431 & 0.973 & 2.732 \\
 \textbf{Cnn14Decision (PANN)} \cite{kong2020panns} & 0.385 & \\
 ERANN \cite{verbitskiy2021eranns} & 0.450 & 0.976 & 2.804 \\
 PSLA \cite{gong2021psla} & 0.444 & 0.975 & 2.778 \\
 AST \cite{gong2021ast} & 0.459 & - & - \\
 PaSST \cite{koutini2021efficient} & 0.471 & - & - \\
 \textbf{HST} & 0.471 & - & - \\
 \bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Anchor accuracy on 381 sound classes}
\label{table:sed}
\begin{tabular}{*{8}{c}}
 \toprule
 & max & 0.1 & 0.2 & 0.5 & 1.0 & 2.0 & 5.0 \\
 \midrule
 CNN Max & 0.6850 & 0.7165 & 0.7266 & 0.7430 & \textbf{0.7507} & 0.7238 & 0.5870  \\
 CNN Attention & 0.6545 & 0.6839 & 0.6916 & 0.7075 & 0.7170 & 0.6981 & 0.5823 \\
 HTS \\
 \bottomrule
\end{tabular}
\end{table}

We now introduce an additive noise model, i.e., $ X = S + N $, which is illustrated in Fig. \ref{fig:cIRM}.
% shows two examples of using cIRM for MSS. 
Here, we focus on each time-frequency bin of STFTs of source, noise, and mixture ($ S(t, f) $, $ N(t, f) $, and $ X(t,f) $, respectively).
% Fig. \ref{fig:cIRM} shows that $ \angle M $ are the phases to be rotated from mixtures to sources. 
Fig. \ref{fig:cIRM} (a) shows an example where the magnitude of cIRM $ |M(t, f)| $ is smaller than 1. This is modelled well in the existing methods where the ranges of complex mask is bound to $[0, 1]$. However, as illustrated in Fig.~\ref{fig:cIRM}~(b), $ |M(t, f)| $ can be larger than 1. As in the figure, this may happen when $S(t, f)$ and $N(t, f)$ are out of phase, since that makes the magnitude of mixture to be smaller than that of (individual) signal. % So that $ |M(t, f)| $ is larger than 1.

To analyze the distribution of cIRMs, we can calculate cIRM $ M $ by:

\begin{equation} \label{eq:cIRM}
\begin{split}
M & = S / X \\
& = \frac{S_{r} + i S_{i}}{X_{r} + i X_{i}} \\
& = \frac{S_{r}X_{r} + S_{i}X_{i} + i(S_{i}X_{r} - S_{r}X_{i})}{X_{r}^{2} + X_{i}^{2}},
\end{split}
\end{equation}

\noindent where $ X_{r} $, $ S_{r} $ are real parts of $ X $ and $ S $ respectively, and $ X_{i} $, $ S_{i} $ are imaginary parts of $ X $ and $ S $ respectively.

\subsubsection{Decoupling Magnitude and Phase for cIRM Estimation}\label{section:decoupling}
% Previous works have shown that estimating phases for MSS is a challenging but important problem \cite{wang2018supervised}. 
Unlike previous works that directly predict real and imaginary parts of masks \cite{choi2018phase, hu2020dccrn}, we propose to decouple the magnitude and phase estimation for MSS so that we can 
optimize their designs separately.
% elaborately design a magnitude prediction model without modifying the phase prediction model. 
As a part of the solution, our system outputs a bounded magnitude mask $ \hat{M}_{\text{mag}} \in \mathbb{R}^{T \times F} $ whose value is in $[0, 1]$. In practice, it is implemented by applying sigmoid function. 
% We denote the magnitude of an estimated mask as $ \hat{M}_{\text{mag}} \in [0, 1]^{T \times F} $, where the magnitude of masks are limited to be between $ 0 $ and $ 1 $ by applying a sigmoid nonlinearity. 
Our system also outputs two more tensors, $ \hat{P}_{\text{r}} \in \mathbb{R}^{T \times F} $ and $ \hat{P}_{\text{i}} \in \mathbb{R}^{T \times F} $. Here, $ \hat{P}_{\text{r}} $ and $ \hat{P}_{\text{i}} $ are real and imaginary parts of $ \angle \hat{M} $, respectively. Then, instead of calculating the angle $ \angle \hat{M} $ directly, we calculate its cosine value $cos \angle \hat{M}$ and sine value $sin \angle \hat{M}$ using $\hat{P}_{\text{r}}$ and $\hat{P}_{\text{i}}$ as follows:
\begin{equation} \label{eq:cos_sin}
\begin{split}
cos \angle \hat{M} & = \hat{P_{\text{r}}} / \sqrt{\hat{P_{\text{r}}}^2 + \hat{P_{\text{i}}}^2} \\
sin \angle \hat{M} & = \hat{P_{\text{i}}} / \sqrt{\hat{P_{\text{r}}}^2 + \hat{P_{\text{i}}}^2}. \\
\end{split}
\end{equation}
\noindent 
% As described in (\ref{eq:cos_sin}), we estimate $cos \angle \hat{M}$ and $sin \angle \hat{M}$ via a real part estimation $\hat{P}_{\text{r}}$, and an imaginary part estimation $\hat{P}_{\text{i}}$. 
Then, we estimate the real and imaginary parts of cIRM by:
\begin{equation} \label{eq:recover_real_imag}
\begin{split}
\hat{M}_{\text{r}} = \hat{M}_{\text{mag}} cos \angle \hat{M} \\
\hat{M}_{\text{i}} = \hat{M}_{\text{mag}} sin \angle \hat{M} \\
\end{split}
\end{equation}
\noindent The cIRM $ \hat{M} = \hat{M}_{r} + j \hat{M}_{i} $ is a complex tensor, and is used to separate a target source from $ X $ by (\ref{eq:mask_mul}). Finally, we apply an inverse STFT to obtain the separated waveform. 

\subsubsection{Combination of Bounded Mask Estimation and Direct Magnitude Prediction}\label{section:attention}
% One limitation of previous cIRM methods \cite{choi2018phase, tan2019complex, wang2018supervised} is that the magnitude of masks are limited. We analyzed the upper bounds of those systems in Table \ref{table:upper_bound}. 
To overcome the limit of the performance discussed in Section~\ref{sec:background}, we propose to combine a bounded mask and direct magnitude prediction to estimate the magnitude of cIRMs. 
The motivation is to use direct magnitude prediction as \textit{residual components}, one that complements the bounded magnitude mask. This is implemented as follow:

\begin{equation} \label{eq:attention}
|\hat{S}| = \text{relu}(\hat{M}_{\text{mag}} \odot |X| + \hat{Q})
\end{equation}

\noindent where 
% $ |\hat{M}| $ is the magnitude of a cIRM bounded between 0 and 1 by a sigmoid non-linearity and 
$ \hat{Q} \in \mathbb{R}^{T \times F} $ is the direct magnitude prediction. In this way, we take the advantages of both of the methods. The ReLU operation ensures that the predicted magnitude is always larger than 0. The estimation of phase $ \angle \hat{M} $ by using $ \hat{P}_{\text{r}} $ and $ \hat{P}_{\text{i}} $ are the same as the one in Section \ref{section:decoupling}. Then, the separated STFT can be obtained by:
\begin{equation} \label{eq:attention_phase}
\hat{S} = |\hat{S}| e^{j (\angle \hat{M} + \angle X)},
\end{equation}
\noindent where $ |\hat{S}| $ is calculated by Eq.~ (\ref{eq:attention}). 

In total, the our proposed MSS system contains four outputs: $ \hat{M}_{\text{mag}} $, $ \hat{Q} $, $ \hat{P}_{\text{r}} $ and $ \hat{P}_{\text{i}} $. All of those outputs share the same backbone architecture and apply an individual linear layer to obtain their outputs. We use sigmoid non-linearity to predict $ \hat{M}_{\text{mag}} $ to ensure they have values between 0 and 1. 
% We apply linear layers to predict $ \hat{Q} $, $ \hat{P}_{\text{r}} $ and $ \hat{P}_{\text{i}} $. 
Fig. \ref{fig:resunet} shows the structure of our proposed method.


\subsubsection{Subband decomposition}

There are two challenges of using the entire STFT as input to a neural network. First, the frequency patterns of different subbands are different \cite{liu2020channel}. For example, low frequency bands mostly contain energy part of sound signals, and high frequency bands have different spectrogram structures. Second, the computation cost of using an entire STFT as input to a neural network is large. To address those problems, we adopt the subband decomposition method to build our general source separation system \cite{liu2020channel}. 

There are two types of subband decomposition. The first type is executed in the time domain. The subband decomposition includes an analysis stage and a synthesis stage. In the analysis stage, a time domain signal $ x $ is analyzed into $ M $ subbands $ \{ x^{(1)}, x^{(2)}, ..., x^{(M)} \} $ using a set of quadrature mirror filterbanks (QMF) followed by a downsampling rate of $ M $. Each $ x^{(m)} $ has the length of $ 1 / M $ of $ x $. Then, the STFT of those subbands are concatenated as a feature map as input to a neural network. The computation cost reduces by a rate of $ 1 \ M $. In the synthesis stage, all separated subband signals $ \{ \hat{s}^{(1)}, \hat{s}^{(2)}, ..., \hat{s}^{(M)} \} $ are upsample by a factor of $ M $ and synthesized back into $ \hat{s} $. 

The second type of subband decomposition is executed on the time-frequency domain. For an input STFT $ X $, the spectrogram is split into $ M $ subbands along the frequency bins: $ \{ X^{(1)}, X^{(2)}, ..., X^{(M)} \} $. The dimension of each $ X^{(m)} $ is $ T \times \frac{F}{M} $. Then, those time-frequency subbands are concatentated along the channel dimension to constitute a bach of data with a shape of $ (B, C \times M, T, \frac{F}{M}) $ as input to a neural network. Finally, the estimated spectrograms $ \{ \hat{S}^{(1)}, \hat{S}^{(2)}, ..., \hat{S}^{(M)} \} $ are concatenated along frequency bins to obtain $ \hat{S} $.
